Derivatives of Stochastic Gradient Descent in parametric optimization

We consider stochastic optimization problems where the objective depends on some parameter, as commonly found in hyperparameter optimization for instance. We investigate the behavior of the derivatives of the iterates of Stochastic Gradient Descent (SGD) with respect to that parameter and show that they are driven by an inexact SGD recursion on a different objective function, perturbed by the convergence of the original SGD. This enables us to establish that the derivatives of SGD converge to the derivative of the solution mapping in terms of mean squared error whenever the objective is strongly convex. Specifically, we demonstrate that with constant step-sizes, these derivatives stabilize within a noise ball centered at the solution derivative, and that with vanishing step-sizes they exhibit $O(\log(k)^2 / k)$ convergence rates. Additionally, we prove exponential convergence in the interpolation regime. Our theoretical findings are illustrated by numerical experiments on synthetic tasks.

==> Parts/alt_setup.tex <==
Given a smooth function $\obj\from\Rd\to\R$, \ac{SGD} seeks minimizers of the optimization problem
\begin{align}
\label{eq:opt_alt}
\tag{Opt}
\min\nolimits_{\point\in\Rd}\;
	\obj(\point)
\end{align}
by relying on updates of the form 
\begin{align}
\new \gets \state - \step \orcl(\state,\sample).
\end{align}


We analyze \ac{SGD} defined by $\initP$ and for $\run = \running$
\begin{align}
\label{eq:SGD_alt}
\tag{SGD}
    \nextP = \currP - \curr[\step] \orcl( \currP , \param ; \next[\sample])
\end{align}
where $(\curr[\learn])$ is a sequence of positive step-sizes and $\orcl$ is a \ac{SFO} gradient oracle. 
We highlight here that the algorithm depends on some parameter $\param \in \params$, possibly encoding a parameter of the function, or of the initialization of the algorithm.

Indeed, the objective here is to minimize in $\point$, the \emph{parametrized} function $\obj$, using \ac{SGD} itself parametrized (out of notational convenience we identify the parameters).

\subsection{Assumptions}


Let us now state our assumptions for the objective function and the black-box oracle providing gradient information for \eqref{eq:SGD_alt} with explicit parameters.

\begin{assumption}
\label{asm:obj_alt}
The function $\obj\from\Rd\times\params\to\R$ satisfies the following conditions for all $\param \in \params$:
\begin{enumerate}
[left=\parindent,label=\upshape(\itshape\alph*\hspace*{.5pt}\upshape)]
% \item
% \label[noref]{asm:obj_alt-lower}
% \emph{Lower-boundedness:}
% 	$\inf \obj > -\infty$
\item
\label[noref]{asm:obj_alt-smooth_alt}
\emph{Smoothness:}
The objective $\obj(\cdot,\param)$ is differentiable and its gradient is $\smooth$-Lipschitz continuous, namely
\begin{align}
\label{eq:LG}
\norm{\derpoint\obj(\point,\param) - \derpoint\obj(\pointalt,\param)}
	\leq \smooth \norm{\point - \pointalt}
\end{align}
for all $\point,\pointalt\in\Rd$.
\item
\label[noref]{asm:obj_alt-strong_alt}
\emph{Strong convexity:}
$\obj(\cdot,\param)$ is $\strong$-strongly convex, \ie $\obj(\cdot,\param) - \frac{\strong}{2} \norm{\cdot}^2$ is convex, for some $\strong>0$. We will denote by $\optP$ the unique minimizer of $\obj(\cdot,\param)$.
\end{enumerate}
\end{assumption}




Regarding the input to \eqref{eq:SGD_alt}, we will assume throughout that the optimizer has access to a stochastic estimate of the gradient of $\obj(\cdot,\param)$ at the point of interest.
Formally, when queried at $\point\in\Rd$, an \ac{SFO} returns a random vector of the form
\begin{align}
\label{eq:SFO_alt}
\tag{SFO}
\orcl(\point,\param;\sample)
	= \derpoint\obj(\point,\param)
		+ \noise(\point,\param;\sample)
\end{align}
where $\sample$ is random, so that $\noise(\point;\sample)$ captures all the noise in the gradient oracle. Note that the dependency in $\point$ is essential to capture query-dependent noise situations which naturally occur in finite-sum settings. 
% This modeling encompass most versions of \eqref{eq:SGD_alt} including minibatch \ac{SGD}, noisy gradient descent, and Langevin Monte Carlo methods.
While it is quite natural to assume that stochastic gradients are unbiased, their variance may not always be bounded. Indeed, as detailed in \cref{asm:noise_alt}\ref{asm:noise_alt-growth}, a dependency in the squared norm of the gradient\footnote{Alternative formulations include the suboptimality or the distance to the optimum, they are all equivalent under \cref{asm:obj_alt}.} has to be present to take into account popular situations such as finite sums of strongly convex functions,  see \eg \citep{bottou2018optimization,gower2019sgd}.


\begin{assumption}
\label{asm:noise_alt}
The observed noise sequence $(\curr[\sample])$ is independent. 
Furthermore, the \acl{SFO}  $\orcl\from\Rd\times\params\times\samples\to\Rd$ satisfies:
\begin{enumerate}
[left=\parindent,label=\upshape(\itshape\alph*\hspace*{.5pt}\upshape)]
\item
\label[noref]{asm:noise_alt-biaiszero}
\emph{No bias:}
	$\ex{\orcl(\point,\param;\sample)} = \derpoint\obj(\point,\param)$ for all $\point\in\Rd, \param\in\params$
\item
\label[noref]{asm:noise_alt-growth}
\emph{Variance control:} 
    $ \ex{\sqnorm{\noise(\point,\param;\sample)} } \leq \noisevar + \varcontrol \sqnorm{\derpoint \obj(\point,\param)}$ for all  $\point\in\Rd, \param\in\params$ 
	%$ \sol\in\sols$;
\end{enumerate}
where $\noisedev, \sdevcontrol \ge 0$.
\end{assumption}



In this setting, we use the natural filtration $(\curr[\filter])$ where for all $\run$,  $\curr[\filter]$ is defined as the $\sigma$-algebra generated by $\initP, \dots, \currP$ (note that $\next[\sample]$ and thus $\orcl( \currP ,\param ; \next[\sample])$ is not $\curr[\filter]$-measurable but $\next[\filter]$-measurable). 
In particular, we have that 
\begin{align}\label{eq:noisemaster_alt}
    \condex{\sqnorm{  \orcl( \currP ,\param ;\next[\sample]) }}[\curr[\filter]] &=  \sqnorm{\derpoint\obj(\currP,\param)} % + 2 \inner{\derpoint\obj(\currP,\param)}{\condex{ \noise( \currP ,\next[\sample])}[\curr[\filter]]}  
    +   \condex{\sqnorm{  \noise( \currP ,\param ;\next[\sample]) }}[\curr[\filter]] \\
    &\leq \noisevar + (1+ \varcontrol) \sqnorm{\derpoint \obj(\currP,\param)}
\end{align}



\subsection{Convergence of \ac{SGD}}

In the flurry of results for the convergence of \ac{SGD}, we will rely on the following proposition which borrows from \citet{gower2019sgd,bottou2018optimization,nguyen2018sgd}.

\begin{proposition}\label{prop:cvsgd_alt}
    Let \cref{asm:obj_alt,asm:noise_alt} hold. Take any $\param\in\params$. Let \eqref{eq:SGD_alt} be run with a stepsize of the form $\curr[\step] = \frac{\const}{(\run+\stepoffset)^\exponent}$ for all $\run$, with $\const>0$, $\exponent\in(0,1]$, and $\stepoffset\in\R_+$ sufficiently large so that $\frac{\const \smooth (1+\varcontrol)}{(\start+\stepoffset)^\exponent}\leq 1$.  
    Then, for any $\run$,
    \begin{align}
    \ex{\sqnorm{\currP - \optP}} = \bigoh\left(\frac{1}{\run^\exponent}\right) .
\end{align}
Furthemore, if $\exponent\in(0.5,1]$, then $\seqinfin{\currP}{\run}$ converges almost surely to $\optP$.
\end{proposition}

\begin{proof}
    
By definition of \eqref{eq:SGD}, we have
\begin{align}
        \sqnorm{ \nextP - \optP } =   \sqnorm{\currP - \optP} +  \curr[\step]^2 \sqnorm{  \orcl( \currP ,\param ; \next[\sample])} - 2\curr[\step] \inner{\currP - \optP}{  \orcl( \currP  ,\param ; \next[\sample])}
\end{align}
and taking the conditional expectation \wrt history, we get using \eqref{eq:noisemaster_alt}
\begin{align}
    \condex{\sqnorm{ \nextP - \optP }}[\curr[\filter]] &\leq 
    \sqnorm{\currP - \optP} +  \curr[\step]^2  \noisevar +  \curr[\step]^2 (1+ \varcontrol) \sqnorm{\derpoint \obj(\currP,\param)}\\
    &~~~~~ - 2\curr[\step] \inner{\currP - \optP}{ \derpoint \obj(\currP,\param)} \\
    %%%%%%%%%%%%%%%%%%%%%%%%
    &\leq  (1 - \curr[\step]\strong) \sqnorm{\currP - \optP} +  \curr[\step]^2  \noisevar +  \curr[\step]^2 (1+ \varcontrol) \sqnorm{\derpoint \obj(\currP,\param)}\\
    &~~~~~ - 2\curr[\step] (\obj(\currP,\param) - \obj(\optP,\param)) \\
    %%%%%%%%%%%%%%%%%%%%%%%%
    &\leq  (1 - \curr[\step]\strong) \sqnorm{\currP - \optP} +  \curr[\step]^2  \noisevar \\
    &~~~~~ +  \curr[\step] \sqnorm{\derpoint \obj(\currP,\param)} \left(  (1+ \varcontrol) \curr[\step] -  \frac{1}{ \smooth} \right) \label{eq:endsgd_alt}
\end{align}
where we used sucessively \cref{asm:noise_alt}, the strong convexity of $\obj(\cdot,\param)$, and the whole \cref{asm:obj_alt} (which implies that $\obj(\point,\param)-\obj(\optP,\param) \geq (2\smooth)^{-1} \sqnorm{  \derpoint \obj(\point,\param) } $ for any $\point$, see \eg \citep[Lem.~3.5]{bubeck2015convex}).

Now, our condition on the stepsize parameters  $\frac{\const \smooth (1+\varcontrol)}{(\start+\stepoffset)^\exponent}\leq 1$  implies that $\curr[\step]$ is smaller than $\frac{1}{\smooth(1+\varcontrol)}$ for all $\run$ and thus that the last term in \eqref{eq:endsgd_alt} is non-positive. By taking full expectation on both sides of \eqref{eq:endsgd_alt}, we obtain that 
\begin{align}
    \ex{\sqnorm{ \nextP - \optP }}
    &\leq  (1 - \curr[\step]\strong) \ex{\sqnorm{\currP - \optP}} +  \curr[\step]^2  \noisevar 
\end{align}
and using that $\curr[\step] = \frac{\const}{(\run+\stepoffset)^\exponent}$ along with \cref{lem:chung1954,lem:chung1954-bis} (depending if $\exponent=1$ or not), we obtain
\begin{align}
    \ex{\sqnorm{\currP - \optP}} = \bigoh\left(\frac{1}{\run^\exponent}\right) 
\end{align}
which shows the first part of our result.


Now, in the case where $\exponent\in(0.5,1]$, $\sum_\run  \curr[\step]^2  \noisevar  < \infty$. Thus, reformulating slightly \eqref{eq:endsgd_alt} to get
\begin{align}
    \condex{\sqnorm{ \nextP - \optP }}[\curr[\filter]] 
    &\leq  \sqnorm{\currP - \optP}  +  \curr[\step]^2  \noisevar  - \curr[\step]\strong \sqnorm{\currP - \optP}
\end{align}
and using \cref{lem:Robbins-Siegmund}, we obtain that with probability one, $\seqinfin{\sqnorm{\currP - \optP}}{\run}$ converges to a random variable and
$\sum_\run \curr[\step]\strong \sqnorm{\currP - \optP} <\infty$.

For the sake of contradiction, assume on this event that for some $\varepsilon$, there is $\runalt$ such that $ \sqnorm{\currP - \optP}\geq \varepsilon$ for all $\run\geq\runalt$. Then, 
\begin{align}
    \sum_\run \curr[\step]\strong \sqnorm{\currP - \optP} \geq  \strong \varepsilon \sum_{\run\geq\runalt} \curr[\step] = +\infty
\end{align}
which is a contradiction. Hence, we have shown that $\seqinfin{\currP}{\run}$ converges almost surely to $\optP$.
\end{proof}

\subsection{Derivating \ac{SGD}}

We now differentiate the iterates of \ac{SGD} with respect to the parameter $\param\in\params$. 

\begin{assumption}
\label{asm:noise_altparam_alt}
The parameters space $\params$ is an open subset of $\R^\dimsalt$. Furthermore,  the function $\obj$ is $C^{2}$-differentiable  and the noise term $\noise(\cdot,\cdot;\sample)$ is $C^1$-differentiable for all $\sample$. 
\end{assumption}

By definition of \eqref{eq:SGD_alt} and our \eqref{eq:SFO_alt} noise model, we get that
\begin{align}
    \nextP = \currP - \curr[\step]   \derpoint\obj(\currP[\point],\param)
		- \curr[\step] \noise(\currP[\point],\param;\next[\sample]).
\end{align}


Now, for any $\param\in\params$ and any $\run\geq\start$, we can define the Jacobian of $\currP$ \wrt $\param$, denoted by $\derparam \currP \in \R^{\dims\times\dimsalt}$.

We get the following recursion:
\begin{align}
   \derparam \nextP &= \derparam \currP  
   - \curr[\step] \dderpoint\obj(\currP[\point],\param)   \derparam \currP 
   - \curr[\step]   \dderpointparam\obj(\currP[\point],\param) \\
   &~~~~~ - \curr[\step]  \derpoint\noise(\currP[\point],\param;\next[\sample])  \derparam \currP
   - \curr[\step]   \derparam \noise(\currP[\point],\param;\next[\sample])
\end{align}

\subsection{From the main text}



\begin{proposition} \label{prop:ratesgd}
    In the setting of \cref{prop:cvsgdnoise}, suppose additionally that  for all $\run$
    \begin{align}
        \curr[\step] = \frac{\const}{(\run+\stepoffset)^\exponent} ~~~~ \text{ and } ~~~~ \curr[\Ebound]^2 = \frac{\constalt}{(\run+\stepoffset)^\exponent}
    \end{align}
    % \begin{itemize}
    %     \item $\curr[\step] = \frac{\const}{(\run+\stepoffset)^\exponent}$
    %     \item  $\curr[\Ebound] = \frac{\constalt}{(\run+\stepoffset)^\exponent}$
    % \end{itemize}
 with $\const>0$, $\constalt\geq0$, $\exponent\in(0,1]$, and $\stepoffset\in\R_+$ sufficiently large so that $\init[\step] \leq   \frac{\strong}{2\smooth^2}$.
    Then, 
    \begin{align}
    \ex{\sqnorm{\curr - \opt}} = \bigoh\left(\frac{1}{\run^\exponent}\right) .
\end{align}
\end{proposition}

\begin{proof}
    Recalling \eqref{eq:SGDRecursion} from the proof of \cref{prop:cvsgdnoise}, we have 
\begin{align}
 \ex{\sqnorm{ \next - \opt }}  
 &\leq \left(1  - \curr[\step] \strong \right) \ex{\sqnorm{\curr - \opt}} +  \curr[\step]^2 \left( 2 \noisevar +  \curr[\Ebound]^2  \right) + 3 \curr[\step] \sqrt{\ex{\sqnorm{\curr - \opt}}} \curr[\Ebound] \\
  &\leq \left(1  - \frac{ \curr[\step] \strong}{2} \right) \ex{\sqnorm{\curr - \opt}} +  \curr[\step]^2 \left( 2 \noisevar +  \curr[\Ebound]^2  \right) + \frac{9 }{2\strong}  \curr[\step]  \curr[\Ebound]^2 \\
  &=  \left(1  - \frac{\const \strong/2}{(\run+\stepoffset)^\exponent}  \right) \ex{\sqnorm{\curr - \opt}} + \frac{2 \const^2 \noisevar}{(\run+\stepoffset)^{2 \exponent}}  +   \frac{9 \const \constalt^2/(2\strong)}{(\run+\stepoffset)^{3\exponent}}   + \frac{\const^2 \constalt^2}{(\run+\stepoffset)^{4\exponent} } 
\end{align}
and thus using \cref{lem:chung1954,lem:chung1954-bis} (depending if $\exponent=1$ or not), we obtain the claimed result.
\end{proof}



% EDOUARD: ending as Franck wrote it.

% \noindent\underline{\emph{No noise ($\curr[\Ebound]=0$ for all $\run$):}} Using that $\curr[\step] = \frac{\const}{(\run+\stepoffset)^\exponent}$ along with \cref{lem:chung1954,lem:chung1954-bis} (depending if $\exponent=1$ or not), we obtain
% \begin{align}
%     \ex{\sqnorm{\curr - \opt}} = \bigoh\left(\frac{1}{\run^\exponent}\right) .
% \end{align}


% Furthermore, in the case where $\exponent\in(0.5,1]$, $\sum_\run  \curr[\step]^2  \noisevar  < \infty$. In the same vein as above, we can use \eqref{eq:endsgd} and our stepsize assumption to get
% \begin{align}
%     \condex{\sqnorm{ \next - \opt }}[\curr[\filter]] 
%     &\leq  \sqnorm{\curr - \opt}  +  2\curr[\step]^2  \noisevar  - \frac{\curr[\step]\strong}{2} \sqnorm{\curr - \opt}
% \end{align}
% and using \cref{lem:Robbins-Siegmund}, we obtain that with probability one, $\seqinfin{\sqnorm{\curr - \opt}}{\run}$ converges to a random variable and
% $\sum_\run \curr[\step]\strong \sqnorm{\curr - \opt} <\infty$.

% For the sake of contradiction, assume on this event that for some $\varepsilon$, there is $\runalt$ such that $ \sqnorm{\curr - \opt}\geq \varepsilon$ for all $\run\geq\runalt$. Then, 
% \begin{align}
%     \sum_\run \curr[\step]\strong \sqnorm{\curr - \opt} \geq  \strong \varepsilon \sum_{\run\geq\runalt} \curr[\step] = +\infty
% \end{align}
% which is a contradiction. Hence, we have shown that $\seqinfin{\curr}{\run}$ converges almost surely to $\opt$.

% \noindent\underline{\emph{Vanishing noise + Bounded iterates ($\curr[\Ebound]=\textfrac{\constalt}{(\run+\stepoffset)^\exponentalt}$ for all $\run$):}} Using that $\curr[\step] = \frac{\const}{(\run+\stepoffset)^\exponent}$ and that the iterates are bounded almost surely, we get that
% \begin{align}
%         \ex{\sqnorm{ \next - \opt }} &\leq \left(1  - \frac{\const\strong/2}{(\run+\stepoffset)^\exponent}   \right) \ex{\sqnorm{\curr - \opt}} + \frac{2 \const^2(\noisevar+\constalt^2)}{(\run+\stepoffset)^{2\exponent} (1+(\run+\stepoffset)^{2\exponentalt} ) }+ \frac{2\const \constalt}{(\run+\stepoffset)^{\exponent+\exponentalt}} \\
%         &\leq \left(1  - \frac{\constaltalt}{(\run+\stepoffset)^\exponent}   \right) \ex{\sqnorm{\curr - \opt}} +  \frac{2\constaltaltalt}{(\run+\stepoffset)^{\exponent+\exponentalt}} \label{eq:sgdVanNoise}
% \end{align}
% then using \cref{lem:chung1954,lem:chung1954-bis} (depending if $\exponent=1$ or not), we obtain
% \begin{align}
%     \ex{\sqnorm{\curr - \opt}} = \bigoh\left(\frac{1}{\run^\exponentalt}\right) .
% \end{align}



% Let us discuss some particular cases for our noise and stepsize sequences. The crucial ingredient here is to characterize the limit of 
% \begin{align}
%     \curr[\delta] \defeq \frac{\sqrt{ \frac{9}{4}\curr[\Ebound]^2 + \strong\curr[\step](\curr[\Ebound]^2 + 2 \noisevar)} +\frac{3}{2} \curr[\Ebound]}{\strong}
% \end{align}


% \begin{itemize}
%     \item \underline{No error:} if $\curr[\Ebound]\equiv 0$, then $\curr[\delta] = \sqrt{ \frac{2 \curr[\step] \noisevar}{\strong}}$. If furthermore, 
%     \begin{itemize}
%         \item $\curr[\step] \equiv \step$, then ${\lim\sup}_{\run \to \infty}  \ex{\sqnorm{ \next - \opt }} \leq  \frac{2 \step \noisevar}{\strong}$ 
%         \item $\curr[\step] \to 0$, then ${\lim\sup}_{\run \to \infty}  \ex{\sqnorm{ \next - \opt }} = 0$
%         \item $\curr[\step] =  \frac{\const}{(\run+\stepoffset)^\exponent}$
%     \end{itemize}
% \end{itemize}



Note that this result is valid if $\constalt=0$ (no additional noise) and that it can be slightly generalized to $\curr[\Ebound]^2 = \frac{\constalt}{(\run+\stepoffset)^\exponentalt}$, in which case it gives $\ex{\sqnorm{\curr - \opt}} = \bigoh\left(\frac{1}{\run^{\min(\exponent,2\exponentalt)}}\right)$.


% \subsection{Convergence of \ac{SGD} with fixed stepsizes}


% \begin{proposition}\label{prop:cvsgdnoisecst}
%     Let \cref{asm:sgd} hold. Let us consider the iterates defined by $\init$ and for all $\run\geq\start$
%     \begin{align}\label{eq:sgdnpoisecst}
%             \next = \curr -  \step \left( \sgradalt( \curr ; \next[\sample]) + \curr[\error] \right)
%     \end{align}
%     where
%     \begin{itemize}
%         \item[\emph{(errors)}] $\seqinfin{\curr[\error]}{\run}$ is a sequence of  $\seqinfin{\curr[\filter]}{\run}$-adapted  random variables such that almost surely $\norm{\curr[\error]} \leq \curr[\Ebound] \leq \Ebound$ where $\seqinfin{\curr[\Ebound]}{\run}$ is a deterministic sequence. Here, $\sample_{\run+1+i}$ is independant of $\curr[\error]$ for all $\run,i \in \N$.
%         \item[\emph{(stepsize)}] $\step \leq  \frac{\strong}{8\smooth^2}$.
%     \end{itemize}

%     Then, depending on $\seqinfin{\curr[\Ebound]}{\run}$, we have
%     \begin{itemize}
%         \item If $\Ebound=0$, then for any $\run$,
%     \begin{align}
%     \ex{\sqnorm{\curr - \opt}} = \left(1-\frac{\step\strong}{2}\right)^{\run-1} \sqnorm{\init-\opt} + \frac{4\step\noisevar}{\strong} 
% \end{align}
%         \item If $\Ebound\geq0$, then $\ex{\sqnorm{\curr - \opt}} $  decreases at least until 
%     \begin{align}
% \ex{\sqnorm{\curr - \opt}} \leq  \frac{32 \Ebound^2}{ \strong^2} + 8 {\step} { \frac{   \noisevar +  \Ebound^2  }{ \strong} }
% \end{align}
%   \item If $\frac{\strong}{4}>\Ebound\geq0$, we can get a rate... 
%     \end{itemize}
% \end{proposition}

% \begin{proof}
% By following the steps of the proofs of \cref{prop:cvsgdnoise} up to \eqref{eq:sgdbeforeB}, we get 
% \begin{align}
%         \ex{\sqnorm{ \next - \opt }}  &\leq \left(1  - \frac{\step \strong}{2}  \right) \ex{\sqnorm{\curr - \opt}} + 2 \step^2 \left(  \noisevar +  \curr[\Ebound]^2  \right) + 2 \step \ex{\norm{\curr - \opt}} \curr[\Ebound] . \label{eq:sgdbeforeBcst}
% \end{align}


% \noindent\underline{\emph{No noise ($\curr[\Ebound]=0$ for all $\run$):}} Using \cref{lem:cst-noise-descent}, we obtain
% \begin{align}
%     \ex{\sqnorm{\curr - \opt}} = \left(1-\frac{\step\strong}{2}\right)^{\run-1} \sqnorm{\init-\opt} + \frac{4\step\noisevar}{\strong} .
% \end{align}

% \noindent\underline{\emph{Bounded noise:}} By Jensen's inequality, we get that 
% \begin{align}
%         \ex{\sqnorm{ \next - \opt }}  &\leq \left(1  - \frac{\step \strong}{2}  \right) \ex{\sqnorm{\curr - \opt}} + 2 \step^2 \left(  \noisevar +  \Ebound^2  \right) + 2 \step \sqrt{\ex{\sqnorm{\curr - \opt}}} \Ebound
% \end{align}
% which is structured as 
% \begin{align}
%        \next[D]^2  &\leq \left(1  -  a \right) \curr[D]^2 + b \curr[D]   + c
% \end{align}
% with $\curr[D] = \sqrt{\ex{\sqnorm{\curr - \opt}}}$ is our non-negative sequence of interest and  $a=\frac{\step \strong}{2}$, $b=2 \step \Ebound$, $c=  2 \step^2 \left(  \noisevar +  \Ebound^2  \right) $ are positive coefficients (except maybe $c$ that could be null).

% We see that $\seqinfin{\curr[D]}{\run}$ is decreasing as long as $a \curr[D]^2 - b \curr[D] - c >0$, \ie as long as 
% \begin{align}
%     \curr[D] \geq  \frac{b+ \sqrt{ac}}{a}   >  \frac{b+ \sqrt{b^2+4ac}}{2a} 
% \end{align}
% where
% \begin{align}
%      \frac{b+ \sqrt{ac}}{a} &=  \frac{2 \step \Ebound + \sqrt{\step \strong   \step^2 \left(  \noisevar +  \Ebound^2  \right)}}{\step \strong/2} \\
%      &=  \frac{4 \Ebound}{ \strong} + 2\sqrt{\step} \sqrt{ \frac{   \noisevar +  \Ebound^2  }{ \strong} }
% \end{align}
% \end{proof}

\section{Technical Lemmas}

In this section we recall several important lemmas that are frequently used in the analysis of stochastic iterative methods.

\begin{lemma}
\label{lem:cst-noise-descent}
Let $\seqinf{\seqitem}{\run}$ be a sequence of real numbers
such that for all $\run$,
\begin{equation}
\notag
    \next[\seqitem]
    \le
    (1-\cons)\curr[\seqitem] + \consalt,
\end{equation}
where $1 > \cons > 0$ and $\consalt > 0$.
Then,
\begin{equation}
\notag
    \seqitem_\run
    \le
    (1-\cons)^{\run-1}\seqitem_1+\frac{\consalt}{\cons}.
\end{equation}
\end{lemma}


\vspace{0.5em}
\begin{lemma}[{{\citet[Lemma~1]{chung1954stochastic}}}]
\label{lem:chung1954}
Let $\seqinf{\seqitem}{\run}$ be a sequence of real numbers
and $\stepoffset\in\N$
such that for all $\run$,
\begin{equation}
\notag
    \label{eq:chung_rec}
    \next[\seqitem]
    \le
    \left(1-\frac{\cons}{\run+\stepoffset}\right)\curr[\seqitem]
    + \frac{\consalt}{(\run+\stepoffset)^{\exponent+1}},
\end{equation}
where $\cons > \exponent > 0$ and $\consalt > 0$.
Then,
\begin{equation}
\notag
    \label{eq:chung_bound}
    \seqitem_\run
    \le
    \frac{\consalt}{\cons-\exponent}\frac{1}{\run^\exponent} + \smalloh\left(\frac{1}{\run^\exponent}\right).
\end{equation}
\end{lemma}

\vspace{0.5em}
\begin{lemma}[{{\citet[Lemma~4]{chung1954stochastic}}}]
\label{lem:chung1954-bis}
Let $\seqinf{\seqitem}{\run}$ be a sequence of real numbers
and $\stepoffset\in\N$
such that for all $\run$,
\begin{equation}
    \notag
    \next[\seqitem]
    \le
    \left(1-\frac{\cons}{(\run+\stepoffset)^{\exponentalt}}\right)\curr[\seqitem]
    + \frac{\consalt}{(\run+\stepoffset)^{\exponent+\exponentalt}},
\end{equation}
where $1 > \exponentalt > 0$ and $\exponent,\cons,\consalt > 0$.
Then,
\begin{equation}
\notag
    \seqitem_\run
    =
    \bigoh\left(\frac{1}{\run^\exponent}\right).
\end{equation}
\end{lemma}


To establish almost sure convergence of the iterates, we rely on the Robbins\textendash Siegmund theorem which apply to non-negative almost-supermatingales.

\vspace{0.5em}
\begin{lemma}[\citet{robbins1971convergence}]
\label{lem:Robbins-Siegmund}
Consider a filtration $\seqinf{\filter}{\run}$ and four non-negative $\seqinf{\filter}{\run}$-adapted
processes $\seqinf{U}{\run}$, $\seqinf{\lambda}{\run}$, $\seqinf{\chi}{\run}$, $\seqinf{\zeta}{\run}$
such that $\sum_\run\curr[\lambda] < \infty$ and $\sum_\run\curr[\chi] < \infty$ with probability one and
$\forall \run\in\N$,
\begin{equation}
    \label{eq:Robbins-Siegmund}
    \condex{\next[U]}[\curr[\filter]]
    \le (1+\curr[\lambda])\curr[U] + \curr[\chi] - \curr[\zeta].
\end{equation}
Then $\seqinf{U}{\run}$ converges almost surely to a random variable $U_\infty$ and
$\sum_\run\curr[\zeta]<\infty$ almost surely.
\end{lemma}

